Accurate Bundle Matching and Generation via Multitask Learning with Partially Shared Parameters

How can we recommend existing bundles to users accurately? How can we generate new tailored bundles for users? Recommending a bundle, or a group of various items, has attracted widespread attention in e-commerce owing to the increased satisfaction of both users and providers. Bundle matching and bundle generation are two representative tasks in bundle recommendation. The bundle matching task is to correctly match existing bundles to users while the bundle generation is to generate new bundles that users would prefer. Although many recent works have developed bundle recommendation models, they fail to achieve high accuracy since they do not handle heterogeneous data effectively and do not learn a method for customized bundle generation. In this paper, we propose BundleMage, an accurate approach for bundle matching and generation. BundleMage effectively mixes user preferences of items and bundles using an adaptive gate technique to achieve high accuracy for the bundle matching. BundleMage also generates a personalized bundle by learning a generation module that exploits a user preference and the characteristic of a given incomplete bundle to be completed. BundleMage further improves its performance using multi-task learning with partially shared parameters. Through extensive experiments, we show that BundleMage achieves up to 6.6% higher nDCG in bundle matching and 6.3x higher nDCG in bundle generation than the best competitors. We also provide qualitative analysis that BundleMage effectively generates bundles considering both the tastes of users and the characteristics of target bundles.

==> 030proposed-old.tex <==


\section{Proposed Method}
\label{sec:proposed_method}
In this section, we propose \method (\methodfullul), a novel approach for personalized bundle recommendation.

\subsection{Overview}
\label{subsec:overview}
We address the following challenges to achieve a high performance of the bundle recommendations:
\begin{itemize}
	\item[C1.] \blue{\textbf{Handling heterogeneous interactions of users.}} \blue{Users have heterogeneous} interactions with items and bundles, both of which are informative for bundle matching. \blue{How can we deal with the heterogeneous interactions} for accurate bundle matching?
%	\item[C1.] \textbf{Understanding user preferences.} It is difficult to understand a user's preference from the user's bundle purchase history since the number of user-bundle interactions are rare in real-world datasets. How can we understand a user's preference?
	\item[C2.] \blue{\textbf{Learning bundle generation mechanism.}} \blue{Bundle generation is a demanding task since the search space of possible bundles is prohibitively unwieldy. Moreover, previous works have not studied to learn bundle generation mechanisms. How can we learn a bundle generation mechanism?}
	\item[C3.] \blue{\textbf{Handling two related but different tasks.}} Bundle matching and generation are related but separate tasks. \blue{How can we effectively train the two tasks to improve their performance?}
%		How can we design an effectively unified architecture for the bundle matching and generation tasks?	
\end{itemize}



The main ideas of \method are summarized as follows:
\begin{itemize}
	\item[I1.] \blue{\textbf{Exploiting users' interactions to predict their bundle interactions.} We train a matching model to predict users' entire bundle interactions using their entire item interactions. It enables us to effectively extract user preferences from the item interactions which contain sufficient information of the users.}
%	\item[I1.] \textbf{Utilizing user-item interactions}, which is more abundant than user-bundle interactions, enables us to better understand each user's preference.
	\item[I2.] \blue{\textbf{Conditional reconstruction for bundle generation.} We learn a generation mechanism by reconstructing an incomplete bundle with user preferences as the condition. It enables us to generate personalized bundles with an incomplete bundle.}
	\item[I3.] \blue{\textbf{Multi-task learning with partially shared parameters.} We train the two models for matching and generation by a multi-task learning manner while sharing parts of embeddings. It enables us to learn the common and separate information of the two tasks and results in achieving high performance on the two tasks simultaneously.}
\end{itemize}

Figure~\ref{fig:overview} shows the overall \blue{architecture} of \method, which consists of \blue{bundle matching module $f_{mat}$ and generation module $f_{gen}$.}
\blue{Given user $u$'s item interactions as a vector $\mathbf{v}_u$, $f_{mat}$ is trained to predict user $u$'s interaction probabilities over bundles.
User $u$'s latent embedding vector $\mathbf{z}_u$, which represents user $u$'s hidden preference, is extracted from her item interactions $\mathbf{v}_u$.}
%The bundle generation module, given a partially masked bundle, predicts the bundle's whole items conditioned to a user who interacted with the bundle;
%the partially masked bundle designates a bundle where some items are treated as unobserved.
%The conditioning operation of the bundle generation module enables it to generate a personalized bundle reflecting the user's preference.
\blue{
Given bundle $b$'s incomplete affiliation as a vector $\ddot{\mathbf{x}}_b$ and user $u$'s embedding vector $\mathbf{z}_u$, the bundle generation module is trained to estimate bundle $b$'s original affiliation probabilities over items;
$\ddot{\mathbf{x}}_b$ is a partially masked vector where a part of nonzero entries are masked as zero from the original vector $\mathbf{x}_b$.
We then find top-$k$ items to be added to the incomplete bundle from the estimated probabilities over items.
The completed bundle can vary depending on target users, even if a given incomplete bundle is the same.
}
The bundle matching and generation modules are trained in a multi-task learning manner while sharing \blue{parts of} item latent embeddings.

In Section~\ref{subsec:motivation_intuition}, we describe our motivations and intuitions for bundle matching and generation.
In Section~\ref{subsec:variational_inference}, we propose a probabilistic graphical model and explain a variational inference based approach to learn the model parameters.
We describe in-depth the unified architecture of bundle matching and generation modules, which is based on neural networks, in Section~\ref{subsec:architecture}.
We explain the objective function and training algorithm of \method in Section~\ref{subsec:training}.

\subsection{Motivation and Intuition}
\label{subsec:motivation_intuition}
\subsubsection{Bundle Matching}
%The objective of bundle matching is to predict bundles that a user will interact with.
%We are given a user's item interactions and bundle interactions, both of which are valuable to predict the bundle matching, since they epitomize the user's preference.
\blue{
The objective of bundle matching is to predict future bundles for a user using her item interactions and bundle interactions.}
Previous works for bundle matching problem utilize the two types of interactions by joint learning of two separate models~\cite{PathakGM17,CaoN0WZC17,ChenL0GZ19}, or by learning on heterogeneous graphs~\cite{ChangG0JL20, VijaikumarSM20}.
%The joint learning has a limitation of requiring meticulous optimization such as balancing the learning rates and handling distinct convergence conditions.
%The learning on heterogeneous graphs has a limitation of necessitating fastidious design such as handling different types of nodes and edges.
%The previous works have failed to achieve high performance on bundle matching due to such limitations.
\blue{However, they have not fully exploited the relationship between a user's item and bundle interactions, which should be dealt with effectively because the two interactions are highly correlated but heterogeneous.}

\blue{
Our intuition for bundle matching is that a user's item interactions contain sufficient information to predict the user's bundle interactions.
In real-world scenarios, users interact with items more frequently than bundles because items are cheaper and more numerous than bundles.
In addition, users' item interactions and bundle interactions are highly correlated;
for instance, users who often purchase pop music are more likely to purchase a bundle consisting of pop music than classical music.
Then, how can we utilize the sufficient information from users' item interactions to predict their bundle interactions?
%Our main idea is to pair up users' item and bundle interactions and train to predict the bundle interactions using the item interactions.
%Our main idea is to extract the preferences of users from their item interactions, and to predict their bundle interactions using the preferences.
Our main idea is to exploit users' entire item interactions for predicting their entire bundle interactions.
After training the model, we are able to predict a user's bundle interactions using her item interactions.
}

%To address such limitation, we exploit a supervised learning scheme, which is a concise yet powerful training fashion when pairs of input and output are given, using a user's item interactions and bundle interactions.
%We construct supervised learning framework to predict the user's bundle interactions using her item interactions for the following reasons.
%The reason for pairing the user's item interactions with bundle interactions is that all users have pairs of item and bundle interactions, and it is effective to extract meaningful information about the user since the user's bundle interactions and item interactions are highly correlated.
%The reason to put the user's item interactions as an input and bundle interactions as an output is that we can directly utilize the framework for our goal of predicting bundles that the user will interact with in the future.

%The reasons are that 1) the user's bundle interactions and item interactions are highly correlated since the both all reflects the user's preference, and 2) we can directly utilize the framework for our goal, which is to predict bundles that the user will purchase in the future.
%For the second reason, it is more reasonable to predict the user's bundle interactions through the user's item interactions because the user often more interacts with items than bundles in a real-world scenario (see Table~\ref{table:datasets} for real-world datasets).

\subsubsection{Bundle Generation}
The objective of bundle generation is to \blue{construct a personalized bundle for a target user.}
\blue{To achieve the goal}, previous works for bundle generation~\cite{PathakGM17,VijaikumarSM20} utilize trained bundle matching models in a greedy manner without training any bundle generation \blue{mechanisms}.
They have limitation of necessitating a heuristic criterion for whether to add new items or remove existing items to a bundle being generated.
%The previous works have failed to achieve high performance on bundle generation since they are lack of efforts on modeling bundle generation process.

%To address such limitation, we model the bundle generation \blue{mechanism} with an assumption as follows.
\blue{Our intuition for bundle generation is that a bundle construction is determined by the preference of a target user and the characteristic of the bundle;}
the characteristics of bundles could vary by domain, \blue{such as genre and provider.}
For instance, assume we want to generate a bundle with "PlayStation" games, and the target user prefers "RPG (Roll Playing Games)".
\blue{We will construct a bundle with "PlayStation" and "RPG" games for the target user.
Then, how can we generate a personalized bundle while considering the target user preference and the bundle characteristic?
Our main idea is to extract bundle characteristic from an incomplete bundle, and to reconstruct the bundle using the bundle characteristic and a target user preference extracted from her item interactions in bundle matching.
After training the model, we are able to generate a personalized bundle for an incomplete bundle and a target user.
%In the training process, we define target users as users who interacted with a bundle with an assumption that the bundle is generated for the target user.
%In the test process, we are able to generate a personalized bundle for a subset of bundle and a target user.
}
%To model the generation \blue{mechanism} with the assumption, we introduce a conditional variational autoencoder~\cite{KingmaMRW14,SohnLY15} based framework, which learns a completion process of a bundle using an incomplete bundle as input and the preference of a target user as a condition.
%The latent embedding of the model extracted from the given incomplete bundle represents the characteristics of the bundle.

%\red{Idea3: multi-task learning with shared parameters (motivation and idea).}

\begin{figure}[t]
\centering
\begin{subfigure}{.49\linewidth}
  \centering
  \includegraphics[width=0.8\linewidth]{./FIG/generation}
  \caption{Generative models.}
  \label{fig:generation}
\end{subfigure}
\begin{subfigure}{.49\linewidth}
  \centering
  \includegraphics[width=0.8\linewidth]{./FIG/approximation}
  \caption{Posterior approximations.}
  \label{fig:approximation}
\end{subfigure}
\caption{
	Probabilistic graphical model representations of bundle recommendation.
}
\label{fig:pgm}
\end{figure}



\subsection{Probabilistic Graphical Model and Variational Inference}
\label{subsec:variational_inference}
%To solve the bundle matching and generation problems, we design a model with two assumptions, which we explained in Section~\ref{subsec:motivation_intuition}, as follows.

\subsubsection{Probabilistic Graphical Model}
\blue{For each user $u$, the probability of bundle matching and generation is defined as $p(\mathbf{r}_u, \mathbf{x}_{b} | u)$, where $\mathbf{r}_u$ is the bundle interaction vector of user $u$, and $\mathbf{x}_{b}$ is the bundle affiliation vector of bundle $b$.
The aim is to train a model to estimate the probability from observable data.
We propose a probabilistic graphical model to embody our intuitions which are stated in Section~\ref{subsec:motivation_intuition}.}

Given the item interactions of users $\mathbf{V}_u$, our goal is to find the optimal parameters $\Theta=\{\rho, \theta, \psi, \phi\}$ that maximize the likelihood $p_\Theta(\mathbf{R}_u,\mathbf{X}_b|\mathbf{V}_u)$ of observed bundle interactions of users $\mathbf{R}_u$ and bundle affiliations $\mathbf{X}_b$.
To tackle the complicated dependencies between the variables, we assume a probabilistic graphical model with latent variables $\mathbf{Z}_u$ and $\mathbf{Z}_b$ as in Figure~\ref{fig:pgm}.
A user's latent variable $\mathbf{Z}_u$ is estimated by $q_\psi$ using the user's item interaction variable $\mathbf{V}_u$.
The user's bundle interaction variable $\mathbf{R}_u$ is estimated by $p_\rho$ using the user's latent variable $\mathbf{Z}_u$.
A bundles's latent variable $\mathbf{Z}_b$ is estimated by $q_\phi$ using a target user's latent variable $\mathbf{Z}_u$ and the bundle's affiliation variable $\mathbf{X}_b$.
The bundle's affiliation variable $\mathbf{X}_b$ is estimated by $p_{\theta}$ using the target user's latent variable $\mathbf{Z}_u$ and the bundle's latent variable $\mathbf{Z}_b$.
We call $p_\rho$ and $p_\theta$ generative models since they model the generation of observed variables $\mathbf{R}_u$ and $\mathbf{X}_b$.
On the other hand, we call $q_\psi$ and $q_\phi$ posterior approximations since they approximate the unobserved latent variables $\mathbf{Z}_u$ and $\mathbf{Z}_b$.


The probabilistic graphical model encompasses two properties as follows.
\begin{property}[Conditional Independence]
	the conditional independence between three variables $\mathbf{V}_u$, $\mathbf{R}_u$, and $\mathbf{X}_b$, given $\mathbf{Z}_u$.
\label{prop:ci}

\noindent We employ Property~\ref{prop:ci} when designing a model since we expect the variable $\mathbf{Z}_u$ has the sufficient information of a user.
We hold the expectation because a user interact with items more often than bundles and the user's item interactions and bundle interactions are highly correlated.
\end{property}
\begin{property}[Conditional Dependence]
	the conditional dependence between two variables $\mathbf{Z}_u$ and $\mathbf{Z}_b$, given $\mathbf{X}_b$.
\label{prop:cd}
\end{property}

\noindent We employ Property~\ref{prop:cd} when designing a model since we expect variable $\mathbf{X}_b$ is affected by variables $\mathbf{Z}_u$ and $\mathbf{Z}_b$.
Note that we assume a bundle's included items are determined by the bundle's characteristic and a target user's preference in Section~\ref{subsec:motivation_intuition}.


\subsubsection{Variational Inference}
The likelihood is represented as\\$p_\Theta(\mathbf{R}_u,\mathbf{X}_b|\mathbf{V}_u)=\mathbb{E}_{\mathbf{Z}_u \sim p(\mathbf{Z}_u|\mathbf{V}_u)}[p_\Theta(\mathbf{R}_u,\mathbf{X}_b|\mathbf{Z}_u,\mathbf{V}_u)]$ using the latent variable $\mathbf{Z}_u$.
However, it includes the intractable expectation over $\mathbf{Z}_u$.
Hence, we detour the problem by maximizing the evidence lower bound (ELBO) as follows:
\begin{multline}
	\log p_\Theta(\mathbf{R}_u,\mathbf{X}_b|\mathbf{V}_u) \geq \mathcal{L}_{\mathbf{R}_u,\mathbf{X}_b}(\Theta) =\\
	\mathbb{E}_{\mathbf{Z}_u \sim q_{\psi}(\mathbf{Z}_u|\mathbf{R}_u,\mathbf{X}_b,\mathbf{V}_u)}[\log p_{\rho,\theta}(\mathbf{R}_u,\mathbf{X}_b|\mathbf{Z}_u,\mathbf{V}_u)]\\
	-D_{\mathrm{KL}}(q_{\psi}(\mathbf{Z}_u|\mathbf{R}_u,\mathbf{X}_b,\mathbf{V}_u)\|p(\mathbf{Z}_u|\mathbf{V}_u)),
\end{multline}
where $\mathcal{L}_{\mathbf{R}_u,\mathbf{X}_b}(\Theta)$ is the ELBO.
Using Property~\ref{prop:ci}, the first term of $\mathcal{L}_{\mathbf{R}_u,\mathbf{X}_b}(\Theta)$ is rewritten as:
\begin{multline}
	\mathbb{E}_{\mathbf{Z}_u \sim q_{\psi}(\mathbf{Z}_u|\mathbf{R}_u,\mathbf{X}_b,\mathbf{V}_u)}[\log p_{\rho,\theta}(\mathbf{R}_u,\mathbf{X}_b|\mathbf{Z}_u,\mathbf{V}_u)]=\\
	\mathbb{E}_{\mathbf{Z}_u \sim q_{\psi}(\mathbf{Z}_u|\cdot)}[\log p_{\rho}(\mathbf{R}_u|\mathbf{Z}_u)] + \mathbb{E}_{\mathbf{Z}_u \sim q_{\psi}(\mathbf{Z}_u|\cdot)}[\log p_{\theta}(\mathbf{X}_b|\mathbf{Z}_u)],
\label{eq:likelihood}
\end{multline}
where $q_{\psi}(\mathbf{Z}_u|\cdot)$ denotes $q_{\psi}(\mathbf{Z}_u|\mathbf{R}_u,\mathbf{X}_b,\mathbf{V}_u)$.
\noindent
%Then, the likelihood is rewritten as $p_\Theta(\mathbf{\bar{X}},\mathbf{X}|\mathbf{U}) = p_\Theta(\mathbf{\bar{X}}|\mathbf{U}) p_\Theta(\mathbf{X}|\mathbf{U})$ using the property $(\mathbf{\bar{X}}\indep\mathbf{X}|\mathbf{U})$ as in Property~\ref{prop:ci}.
We call the first term and second term in Equation~\eqref{eq:likelihood} as bundle matching reconstruction and bundle generation reconstruction, respectively.
%We call $p_\Theta(\mathbf{X}|\mathbf{U})$ as bundle generation likelihood, and $p_\Theta(\mathbf{\bar{X}}|\mathbf{U})$ as bundle matching likelihood.
%The second term of $\mathcal{L}(\Theta)$ regularizes $q_{\phi}(\mathbf{Z}_\mathbf{U}|\mathbf{X},\mathbf{\bar{X}},\mathbf{U})$ to be close to $p(\mathbf{Z}_\mathbf{U}|\mathbf{U})$.
%We explain the bundle matching likelihood and bundle generation likelihood, respectively, in the following paragraphs in details.

%\textbf{Bundle matching likelihood.}
%To handle the complicated dependencies of $\mathbf{\bar{X}}$, we introduce a latent variable $\mathbf{Z_\mathbf{U}}$ and represent the bundle matching likelihood as $p_{\Theta}(\mathbf{\bar{X}}|\mathbf{U})=\mathbb{E}_{\mathbf{Z_{\mathbf{U}}} \sim p(\mathbf{Z_{\mathbf{U}}}|\mathbf{U})}[p_\Theta(\mathbf{\bar{X}}|\mathbf{Z_{\mathbf{U}}},\mathbf{U})]$.
%We assume $(\mathbf{\bar{X}}\indep\mathbf{U}|\mathbf{Z_\mathbf{U}})$ meaning the conditional independence between $\mathbf{\bar{X}}$ and $\mathbf{U}$ given $\mathbf{Z_{\mathbf{U}}}$, expecting $\mathbf{Z_{\mathbf{U}}}$ has the sufficient information to generate the bundle set $\mathbf{\bar{X}}$.
%Then, the ELBO of the bundle matching log-likelihood is written as follows:
%\begin{multline}
%	\log p_\Theta(\mathbf{\bar{X}}|\mathbf{U}) \geq \mathcal{L}(\Theta) =\\
%	\mathbb{E}_{\mathbf{Z_{\mathbf{U}}}\sim q_{\phi}(\mathbf{Z_{\mathbf{U}}}|\mathbf{\bar{X}},\mathbf{U})}[\log p_\theta(\mathbf{\bar{X}}|\mathbf{Z}_\mathbf{U},\mathbf{U})]
%	-D_{\mathrm{KL}}(q_{\phi}(\mathbf{Z}_\mathbf{U}|\mathbf{\bar{X}},\mathbf{U})\|p(\mathbf{Z}_\mathbf{U}|\mathbf{U})),
%\end{multline}
%where $\mathcal{L}(\Theta)$ is the ELBO. 

%\textbf{Bundle generation likelihood.}
%Analogous to the bundle matching likelihood, we introduce a latent variable $\mathbf{Z_{\mathbf{B}}}$ and represent the bundle generation likelihood as $p_{\Theta}(\mathbf{X}|\mathbf{U})=\mathbb{E}_{\mathbf{Z_{\mathbf{B}}} \sim p(\mathbf{Z_{\mathbf{B}}}|\mathbf{U})}[p_\Theta(\mathbf{X}|\mathbf{Z_{\mathbf{B}}},\mathbf{U})]$.
%We propose a Conditional Variational Autoencoder (CVAE) where the bundle generation likelihood is conditioned on the user information $\mathbf{U}$.
%By the assumption that $\mathbf{Z}_{\mathbf{U}}$ has the sufficient information to generate $\mathbf{U}$, the ELBO of the bundle generation log-likelihood is written as follows:
%\begin{multline}
%	\log p_\Theta(\mathbf{X}|\mathbf{Z}_{\mathbf{U}}) \geq \mathcal{L}(\Theta) =\\
%	\mathbb{E}_{\mathbf{Z}_\mathbf{B} \sim q_{\phi}(\mathbf{Z}_\mathbf{B}|\mathbf{X},\mathbf{Z}_\mathbf{U})}[\log p_\theta(\mathbf{X}|\mathbf{Z}_\mathbf{B},\mathbf{Z}_\mathbf{U})]\\
%	-D_{\mathrm{KL}}(q_{\phi}(\mathbf{Z}_\mathbf{B}|\mathbf{X},\mathbf{Z}_\mathbf{U})\|p(\mathbf{Z}|\mathbf{Z}_\mathbf{U})),
%\end{multline}
%where $\mathcal{L}(\Theta)$ is the ELBO.

To generate a personalized bundle using user information as assumed in Property~\ref{prop:cd}, we formalize the ELBO of the bundle generation with latent variable $\mathbf{Z}_b$ and condition $\mathbf{Z}_u$ as follows:
\begin{multline}
\label{eq:bundle_gen}
	\log p_\Theta(\mathbf{X}_b|\mathbf{Z}_u) \geq \mathcal{L}_{\mathbf{X}_b}(\Theta) =\\
	\mathbb{E}_{\mathbf{Z}_b \sim q_{\phi}(\mathbf{Z}_b|\mathbf{X}_b,\mathbf{Z}_u)}[\log p_\theta(\mathbf{X}_b|\mathbf{Z}_b,\mathbf{Z}_u)]\\
	-D_{\mathrm{KL}}(q_{\phi}(\mathbf{Z}_b|\mathbf{X}_b,\mathbf{Z}_u)\|p(\mathbf{Z}_b|\mathbf{Z}_u)),
\end{multline}
where $\mathcal{L}_{\mathbf{X}_b}(\Theta)$ is the ELBO of the bundle generation.
In Equation~\eqref{eq:bundle_gen}, the first term measure how well the observed bundle affiliation $\mathbf{X}_b$ is generated using bundle latent variable $\mathbf{Z}_b$ that is sampled from $q_\phi$ with a condition of user latent variable $\mathbf{Z}_u$.
The second term regularizes $q_{\phi}(\mathbf{Z}_b|\mathbf{X}_b,\mathbf{Z}_u)$ to be close to the prior $p(\mathbf{Z}_b|\mathbf{Z}_u)$.

At this end, our goal is to find the optimal parameters $\Theta$ that maximize the lower bound of the likelihood as follows:
\begin{multline}
\label{eq:objective}
	\log p_\Theta(\mathbf{R}_u,\mathbf{X}_b|\mathbf{V}_u)\geq\\
	\mathbb{E}_{\mathbf{Z}_u \sim q_{\psi}(\mathbf{Z}_u|\cdot)}[\log p_{\rho}(\mathbf{R}_u|\mathbf{Z}_u)] - D_{\mathrm{KL}}(q_{\psi}(\mathbf{Z}_u|\cdot)\|p(\mathbf{Z}_u|\mathbf{V}_u)) \\
	+ \mathbb{E}_{\mathbf{Z}_u \sim q_{\psi}(\mathbf{Z}_u|\cdot)}[\mathcal{L}_{\mathbf{X}_b}(\Theta)],
\end{multline}
where $q_{\psi}(\mathbf{Z}_u|\cdot)$ denotes $q_{\psi}(\mathbf{Z}_u|\mathbf{R}_u,\mathbf{X}_b,\mathbf{V}_u)$.
In Equation~\eqref{eq:objective}, the first term in Equation~\eqref{eq:objective} measures how well the observed bundle interaction $\mathbf{R}_u$ is generated using user latent factor $\mathbf{Z}_u$ that is sampled from $q_{\psi}$.
%The second term measures how well the observed bundle affiliation $\mathbf{X}_B$ is generated using user latent factor $\mathbf{Z}_U$.
The second term regularizes $q_{\psi}(\mathbf{Z}_u|\cdot)$ to be close to the prior $p(\mathbf{Z}_u|\mathbf{V}_u)$.
After finding the optimal parameters $\Theta$, we are able to match the existing bundles and generate personalized bundles for a user given her item interactions.

\textbf{Prior assumption.}
We assume prior $p(\mathbf{Z}_b|\mathbf{Z}_u)$ in Equation~\eqref{eq:bundle_gen} and prior $p(\mathbf{Z}_u|\mathbf{V}_u)$ in Equation~\eqref{eq:objective} as multivariate Gaussian distributions.
Specifically, we use
This is because the multivariate Gaussian distribution has been studied that it represents the real-world data effectively in previous works for various domains such as image representation~\cite{KingmaW13,KipfW16a}, graph representation~\cite{RezendeMW14}, and collaborative filtering~\cite{LiangKHJ18}.

\textbf{Reparameterization trick.}
In a straightforward approach, Equation~\eqref{eq:objective} is estimated by sampling $\mathbf{Z}_u$ and $\mathbf{Z}_b$ from $q_\psi$ and $q_\phi$, respectively, and optimize the parameters through gradient ascents.
However, it is not trivial to handle the gradients with respect to parameters $\psi$ and $\phi$ via the sampling process.
Using reparameterization trick~\cite{KingmaW13}, which detour this pitfall, we sample $\epsilon_u\sim\mathcal{N}(0,\mathbf{I}_d)$ and reparameterize $\mathbf{Z}_u=\mu_{\psi}(\mathbf{V}_u)+\epsilon_u\odot\sigma_{\psi}(\mathbf{V}_u)$, where $d$ is the dimensionality of latent variable $\mathbf{Z}_u$, and $\mu_\psi$, $\sigma_\psi$ are parameterized functions in $q_\psi$.
In a similar way, we reparameterize $\mathbf{Z}_b=\mu_{\phi}(\mathbf{X}_b,\mathbf{Z}_u)+\epsilon_b\odot\sigma_{\phi}(\mathbf{X}_b,\mathbf{Z}_u)$, where $\epsilon_b\sim\mathcal{N}(0,\mathbf{I}_d)$ is a sampled noise, and $\mu_\phi$, $\sigma_\phi$ are parameterized functions of $q_\phi$.
By virtue of the reparameterization trick, the stochasticities in the sampling processes are isolated and the gradients with respect to the parameters can be back-propagated through sampled $\mathbf{Z}_u$ and $\mathbf{Z}_b$.


%To handle the complicated dependencies of data, we introduce a latent variable $\mathbf{Z}$ and represent the likelihood as $p_\Theta(\mathbf{X},\mathbf{\bar{X}}|\mathbf{U})=\mathbb{E}_{\mathbf{Z} \sim p(\mathbf{Z}|\mathbf{U})}[p_\Theta(\mathbf{X},\mathbf{\bar{X}}|\mathbf{Z},\mathbf{U})]$.
%However, it includes the intractable expectation over $\mathbf{Z}$.
%Hence, we maximize the evidence lower bound (ELBO) as follows:
%\begin{multline}
%	\log p_\Theta(\mathbf{X},\mathbf{\bar{X}}|\mathbf{U}) \geq \mathcal{L}(\Theta) =\\
%	\mathbb{E}_{\mathbf{Z}\sim q_{\phi}(\mathbf{Z}|\mathbf{X},\mathbf{\bar{X}},\mathbf{U})}[\log p_\theta(\mathbf{X},\mathbf{\bar{X}}|\mathbf{Z},\mathbf{U})]\\
%	-D_{\mathrm{KL}}(q_{\phi}(\mathbf{Z}|\mathbf{X},\mathbf{\bar{X}},\mathbf{U})\|p(\mathbf{Z}|\mathbf{U})),
%\end{multline}
%where $\mathcal{L}(\Theta)$ is the ELBO.
%We assume $\mathbf{U}$ has the sufficient information to generate the item set $\mathbf{X}$ and bundle set $\mathbf{\bar{X}}$.
%To this end, we propose a probabilistic graphical model which encompasses the following properties.
%\begin{property}
%	$(\mathbf{X}\indep\mathbf{\bar{X}}|\mathbf{U})$ meaning the conditional independence between $\mathbf{X}$ and $\mathbf{\bar{X}}$ given $\mathbf{U}$.
%\end{property}
%\red{
%\begin{property}
%	$q_{\phi}(\mathbf{Z}|\mathbf{X},\mathbf{\bar{X}},\mathbf{U})=q_{\phi}(\mathbf{Z}|\mathbf{U})$ indicating that the posterior is approximated with the evidence $\mathbf{U}$ without $\mathbf{X}$ and $\mathbf{\bar{X}}$.
%\end{property}}
%As a result, the ELBO is rewritten as follows:
%\begin{multline}
%	\mathcal{L}(\Theta) =
%	\mathbb{E}_{\mathbf{Z}\sim q_{\phi}(\mathbf{Z}|\mathbf{U})}[\log p_\theta(\mathbf{X}|\mathbf{Z}) + \log p_{\bar{\theta}}(\mathbf{\bar{X}}|\mathbf{Z})]\\
%	-D_{\mathrm{KL}}(q_{\phi}(\mathbf{Z}|\mathbf{U})\|p(\mathbf{Z}|\mathbf{U})).
%\label{eq:elbo}
%\end{multline}
%The first term in Equation~(\ref{eq:elbo}) measures how well the observed item set $\mathbf{X}$ and bundle set $\mathbf{\bar{X}}$ are generated from the latent variable $\mathbf{Z}$.
%The second term in Equation~(\ref{eq:elbo}) regularizes the parametrized distribution $q_\phi(\mathbf{Z}|\mathbf{U})$ to be close to the prior $p(\mathbf{Z}|\mathbf{U})$.
%\red{Thus, maximizing Equation~(\ref{eq:elbo})}
%
%\red{
%\begin{multline}
%	\mathcal{L}(\Theta) =
%	\mathbb{E}_{\mathbf{Z}\sim q_{\phi}(\mathbf{Z}|\mathbf{\bar{X}},\mathbf{U})}[\log p_\theta(\mathbf{X}|\mathbf{Z},\mathbf{U}) + \log p_{\bar{\theta}}(\mathbf{\bar{X}}|\mathbf{Z},\mathbf{U})]\\
%	-D_{\mathrm{KL}}(q_{\phi}(\mathbf{Z}|\mathbf{\bar{X}},\mathbf{U})\|p(\mathbf{Z}|\mathbf{U})).
%\label{eq:elbo}
%\end{multline}}

\subsection{Architecture}
\label{subsec:architecture}
In this section, we describe the architecture of \method, which is depicted in Figure~\ref{fig:overview}.
\method consists of two modules, bundle matching module $f_{mat}$ and bundle generation module $f_{gen}$.
We describe the modules $f_{mat}$ and $f_{gen}$ in Sections~\ref{subsubsec:bundle_matching} and~\ref{subsubsec:bundle_generation}, respectively.

\subsubsection{Bundle Matching Module}
\label{subsubsec:bundle_matching}
The bundle matching module $f_{mat}$ aims to predict user $u$'s bundle interactions $\mathbf{R}_u$ using her item interactions $\mathbf{V}_u$.
The module $f_{mat}$ consists of matching encoder $f_{\psi}$ and matching decoder $f_{\rho}$ to model $q_\psi(\mathbf{Z}_u|\mathbf{V}_u)$ and $p_\rho(\mathbf{R}_u|\mathbf{Z}_u)$, respectively.

\textbf{Matching encoder.}
The matching encoder $f_{\psi}$ extracts a user's latent representation $\mathbf{Z}_u$ from her bundle interaction $\mathbf{V}_u$.
%$f_{\psi}$ needs to estimate the mean $\mu_u$ and log-variance $\sigma_{u}$ of the prior $p(\mathbf{Z}_u|\mathbf{V}_u)$, since we assume the prior as a multivariate Gaussian distribution as stated in Section~\ref{subsec:variational_inference}.
We propose an architecture of the matching encoder $f_{\psi}: \mathbb{R}^{N_i} \mapsto \mathbb{R}^{d}$ which estimates the user latent representation $\mathbf{Z}_u$ as follows:
\begin{equation}
\label{eq:matching_encoder}
\begin{multlined}
	\mathbf{Z}_u = f_{\psi}(\mathbf{V}_u) = \mu_{u}+\epsilon_u\odot\sigma_{u}, \text{where}\\
	[\mu_u, \sigma_u] = FNN_{\psi} \left(\frac{\mathbf{V}_u^\top \mathbf{E}^{\psi}}{|\mathbf{V}_u|}\right).
\end{multlined}
\end{equation}
In Equation~\eqref{eq:matching_encoder}, $\epsilon_u\sim\mathcal{N}(0,\mathbf{I}_d)$ is a sampled noise, $\odot$ indicates the element-wise product, $\mathbf{E}^{\psi}\in\mathbb{R}^{N_i\times d_{e}}$ is a trainable matrix with the dimensionality of embedding $d_{e}$, $FNN_{\psi}: \mathbb{R}^{d_e} \mapsto \mathbb{R}^{2d}$ is a fully connected neural network, and bracket $[\cdot]$ denotes a concatenation.
$f_{\psi}$ obtains a low dimensional latent vector by averaging embedding vectors of items that have non-zero values in $\mathbf{V}_u$, and feed it into $FNN_{\psi}$ which extracts mean $\mu_u$ and log-covariance $\sigma_u$ at once.
Finally, $f_{\psi}$ obtains the user latent representation $\mathbf{Z}_u$ by the reparameterization trick~\cite{KingmaW13} which is stated in Section~\ref{subsec:variational_inference}.
$\mathbf{E}^{\psi}_i$, $i$'th row in $\mathbf{E}^{\psi}$, is trained to represent item $i$ for the matching encoder.
%We then adopt a multi-layered fully connected neural network as $fnn(\frac{\mathbf{V}_u^\top \mathbf{E}^{item}}{|\mathbf{V}_u|})$, where the hyperbolic tangent is applied as an activation function and dropout~\cite{SrivastavaHKSS14} is used for the generalized performance.
%In other words, the matching encoder takes a user's item interactions $\mathbf{V}_u$ as an input and outputs the mean and log-variance as $f_{mat}^{en}(\mathbf{V}_u)=fnn(\frac{\mathbf{V}_u^\top \mathbf{E}^{item}}{|\mathbf{V}_u|})=(\mu_u, \sigma_u)$.

\textbf{Matching decoder.}
The matching decoder $f_{\rho}$ estimates a user's bundle interactions $\mathbf{R}_u$ from her latent representation $\mathbf{Z}_u$ which is obtained in Equation~\eqref{eq:matching_encoder}.
It is crucial to predict the probability of user $u$'s interaction with bundles, $\pi_{\mathcal{B}}(u)$, so that we rank the order of the bundles.
We thus design $f_{\rho}$ to predict user $u$'s interaction probability over bundles, $\pi_{\mathcal{B}}(u)$, instead of the values of elements in $\mathbf{R}_u$.
We propose an architecture of the matching decoder $f_{\rho}: \mathbb{R}^d \mapsto \mathbb{R}^{N_b}$ as follows:
\begin{equation}
\label{eq:pi_mat}
	\pi_{\mathcal{B}}(u) = f_{\rho}(\mathbf{Z}_u) = Softmax(\mathbf{E}^{bundle} FNN_{\rho}(\mathbf{Z}_u)),
\end{equation}
where $\mathbf{E}^{bundle} \in \mathbb{R}^{N_b \times d_e}$ is an embedding matrix of bundles, $FNN_{\rho}: \mathbb{R}^{d} \mapsto \mathbb{R}^{d_e}$ is a fully connected neural network, and $Softmax(\cdot)$ is the softmax function.
To achieve high performance in bundle matching, we propose to obtain bundle $b$'s embedding vector $\mathbf{E}^{bundle}_b$ using embedding vectors of items which included in the bundle $b$ as follows:
\begin{equation}
\label{eq:bundle_emb}
	\mathbf{E}^{bundle}_b = \frac{\mathbf{X}_b^{\top}\mathbf{E}^{\rho}}{|\mathbf{X}_b|},
\end{equation}
where $\mathbf{E}^{\rho}\in \mathbb{R}^{N_i\times d_e}$ is a trainable matrix.
We expect that Equation~\eqref{eq:bundle_emb} gives generalization performance gain since even different bundles will inevitably have similar embedding vectors if they consist of similar items.
This is especially effective when the number of unique bundles is large.
%In the third term in Equation~\ref{eq:pi_mat}, $\pi_{mat}(\mathbf{Z}_u)$ indicates the bundle matching probability of user $u$ over all bundles when the user's latent representation $\mathbf{Z}_u$ is given.
In Equation~\eqref{eq:pi_mat}, the user latent representation $\mathbf{Z}_u$ is fed into $FNN_{\rho}$ and the output is used for obtaining scores between all bundles and user $u$.
Finally, a matching probability $\pi_{\mathcal{B}}(u)$ is obtained by the softmax function using the scores.
Note that $\mathbf{E}^{bundle}_b$, $b$'th row in $\mathbf{E}^{bundle}$, represents bundle $b$ for the matching decoder.
%We first adopt a multi-layered fully connected neural network as $fnn(\mathbf{Z}_u)$.
%The matching decoder takes a user's latent representation as an input and outputs the user's bundle interactions as $f_{mat}^{de}(\mathbf{Z}_u)=\mathbf{R}_u$.
%Similar to $f_{mat}^{en}(\cdot)$, we use the hyperbolic tangent and dropout in $f_{mat}^{de}(\cdot)$.
%
%The bundle matching module $f_{mat}$, which is modeled as $p_{\Theta}(\mathbf{R}_U|\mathbf{V}_U)$, aims to predict a user's bundle interactions using the user's item interactions.
%$f_{mat}$ includes the parameterized functions $q_{\psi}(\mathbf{Z}_U|\mathbf{R}_U,\mathbf{X}_B,\mathbf{V}_U)$ and $p_{\rho}(\mathbf{R}_U|\mathbf{Z}_U)$.
%To model $f_{mat}$, we adopt Variational Autoencoder~\cite{KingmaW13}, which has been proven to be effective in supervised learning~\cite{KameokaLIM19} as well as unsupervised learning~\cite{DilokthanakulMG16,HsuZG17,LiangKHJ18}, where $q_{\psi}(\mathbf{Z}_U|\mathbf{R}_U,\mathbf{X}_B,\mathbf{V}_U)$ and $p_{\rho}(\mathbf{R}_U|\mathbf{Z}_U)$ are an encoder and a decoder, respectively.
%\textbf{Encoder network.}
%The encoder of $f_{mat}$, $f_{mat}^{(e)}:\mathbb{R}^{N_i}\mapsto\mathbb{R}^d$ where $N_i$ is the number of items and $d$ is the dimensionality of latent embeddings, aims to extract user $u$'s meaningful latent embedding vector $z_u\in\mathbb{R}^d$ using the user's item interaction vector $\mathbf{R}_u\in\mathbb{R}^{N_i}$.
%Following a recent work~\cite{LiangKHJ18}, we adopt a multi-layered fully connected neural network for $f_{mat}^{(e)}$ where the hyperbolic tangent (Tanh) is applied as an activation function and dropout is used for the generalized performance.
%Since we assume the prior of bundle matching follows the Gaussian distribution, $f_{mat}^{(e)}$ first 
%Since we choose $f_{mat}^{(e)}$ 

\subsubsection{Bundle Generation Module}
\label{subsubsec:bundle_generation}
The bundle generation module $f_{gen}$ aims to predict bundle $b$'s affiliations $\mathbf{X}_b$ using a target user $u$'s latent representation $\mathbf{Z}_u$.
%a partially masked item affiliation $\ddot{\mathbf{X}}_b$
The module $f_{gen}$ consists of generation encoder $f_{\phi}$ and generation decoder $f_{\theta}$ to model $q_\phi(\mathbf{Z}_b|\mathbf{X}_b,\mathbf{Z}_u)$ and $p_\theta(\mathbf{X}_b|\mathbf{Z}_b,\mathbf{Z}_u)$, respectively.
We propose to adopt a Conditional Variational Autoencoder (CVAE)~\cite{KingmaMRW14,SohnLY15} in our setting since it has been studied to effectively learn a generation process using a given condition.
For $f_{\phi}$, we revise the CVAE to estimate bundle $b$'s latent representation $\mathbf{Z}_b$ using the partially masked item affiliation $\ddot{\mathbf{X}}_b$ instead of the original item affiliation $\mathbf{X}_b$.
This idea entails two key advantages as follows.
First, we are able to utilize the model in bundle generation task which is defined in Problem~\ref{problem:bundle_generation}.
In the bundle generation task, we aim to complete an incomplete bundle for a target user.
Second, an autoencoder model shows robust performance on widespread machine learning tasks when it is trained to reconstruct an output using a partially destructed input~\cite{VincentLBM08}.
For instance, a denoising autoencoder~\cite{VincentLLBM10}, which reconstruct a destructed image, effectively learns the latent representation of the image and further reconstruct the image accurately.
We thus expect a robust bundle generation performance by using the partially masked item affiliation $\ddot{\mathbf{X}}_b$ as an input.
In summary, we represent the incomplete bundle as a partially masked item affiliation vector $\ddot{\mathbf{X}}_b$, and $f_{\phi}$ extracts its latent representation using a condition of target user's latent representation $\mathbf{Z}_u$ as $q_\phi(\mathbf{Z}_b|\ddot{\mathbf{X}}_b,\mathbf{Z}_u)$.
After that, $f_{\theta}$ estimates the original item affiliation vector $\mathbf{X}_b$ as $p_\theta(\mathbf{X}_b|\mathbf{Z}_b,\mathbf{Z}_u)$ to complete the incomplete bundle affiliation $\ddot{\mathbf{X}}_b$.

\textbf{Generation encoder.}
%$f_{\phi}$ needs to handle two latent vectors $\mathbf{Z}_b$ and $\mathbf{Z}_u$ as inputs.
%Analogous to the matching encoder, $f_{\phi}$ needs to estimate the mean $\mu_b$ and log-variance $\sigma_{b}$ of the Gaussian prior $p(\mathbf{Z}_b|\mathbf{Z}_u)$.
The generation encoder $f_{\phi}$ extracts bundle $b$'s latent representation $\mathbf{Z}_b$ from its partially masked item affiliation $\ddot{\mathbf{X}}_b$ and target user $u$'s latent representation $\mathbf{Z}_u$.
We propose an architecture of the generation encoder $f_{\phi}: \mathbb{R}^{d+N_i}\mapsto \mathbb{R}^{d}$ as follows:
\begin{equation}
\label{eq:generation_encoder}
\begin{multlined}
	\mathbf{Z}_b = f_{\phi}(\ddot{\mathbf{X}}_b,\mathbf{Z}_u) = \mu_{b}+\epsilon_b\odot\sigma_{b}, \text{where}\\
	[\mu_b, \sigma_b] = FNN_{\phi}\left([\frac{\ddot{\mathbf{X}}_b^\top \mathbf{E}^{\phi}}{|\ddot{\mathbf{X}}_b|}, \mathbf{Z}_u]\right).
\end{multlined}
\end{equation}
In Equation~\eqref{eq:generation_encoder}, $\epsilon_b\sim\mathcal{N}(0,\mathbf{I}_d)$ is a sampled noise, $\odot$ indicates the element-wise product, $\mathbf{E}^{\phi}\in \mathbb{R}^{N_i\times d_e}$ is a trainable matrix, $FNN_{\phi}: \mathbb{R}^{d+d_e}\mapsto \mathbb{R}^{2d}$ is a fully connected neural network, and bracket $[\cdot]$ denotes a concatenation.
$f_{\phi}$ obtains a low dimensional latent vector by averaging embedding vectors of items that have non-zero values in $\ddot{\mathbf{X}}_b$.
Then, $f_{\phi}$ concatenates the averaged embedding vectors with the user latent vector $\mathbf{Z}_u$ and feed it into $fnn_{\phi}$ to obtain $\mu_b$ and $\sigma_b$ at once.
Finally, $f_{\phi}$ obtains the bundle latent representation $\mathbf{Z}_u$ using the reparameterization trick.
Note that $\mathbf{E}_i^{\phi}$, $i$'th row in $\mathbf{E}^{\phi}$, is trained to represent item $i$ for the generation encoder.

\textbf{Generation decoder.}
The generation decoder $f_{\theta}$ estimates bundle $b$'s item affiliation $\mathbf{X}_b$ from the bundle's latent representation $\mathbf{Z}_b$ with target user $u$'s latent representation $\mathbf{Z}_u$ as a condition.
Analogous to the matching decoder, we design $f_{\theta}$ to predict bundle $b$'s affiliation probability over items, $\pi_{\mathcal{I}}(b,u)$, instead of the values of elements in $\mathbf{X}_b$.
We propose an architecture of the generation decoder $f_{\theta}: \mathbb{R}^{d}\mapsto \mathbb{R}^{N_i}$ as follows:
\begin{equation}
\label{eq:pi_gen}
	\pi_{\mathcal{I}}(b,u) = f_{\theta}(\mathbf{Z}_b,\mathbf{Z}_u) = Softmax(\mathbf{E}^{\theta} FNN_{\theta}([\mathbf{Z}_b,\mathbf{Z}_u])),
\end{equation}
where $\mathbf{E}^{\theta}\in \mathbb{R}^{N_i\times d_e}$ is a trainable matrix, $FNN_{\theta}: \mathbb{R}^{2d}\mapsto \mathbb{R}^{d_e}$ is a fully connected neural network, and $Softmax(\cdot)$ is the softmax function.
%In Equation~\ref{eq:pi_gen}, $\pi_{gen}(\mathbf{Z}_u,\mathbf{Z}_b)$ indicates the bundle generation probability of bundle $b$ over all items when the target user's latent representation $\mathbf{Z}_u$ is given.
In Equation~\eqref{eq:pi_gen}, the concatenated vector of $\mathbf{Z}_u$ and $\mathbf{Z}_b$ is fed into $fnn_{\theta}$ and the output is used for obtaining scores for all items;
Finally, a generation probability $\pi_{\mathcal{I}}(b,u)$ is obtained by the softmax function using the scores.
Note that $\mathbf{E}^{\theta}_i$, $i$'th row in $\mathbf{E}^{\theta}$, is trained to represent item $i$ for the generation decoder.

\subsubsection{Parameter Sharing}
\label{subsubsec:parameter_sharing}
Parameter sharing technique is broadly studied and it is incentivized in multi-task learning since it bestows an advantage of impressive performance~\cite{Caruana93,LiWLS22}.
We thus propose to share item embeddings of \method to achieve high performance on bundle matching and generation simutaneously.
Specifically, for item $i$, we propose to share half of $\mathbf{E}^{\psi}_i$, $\mathbf{E}^{\rho}_i$, $\mathbf{E}^{\phi}_i$, and $\mathbf{E}^{\theta}_i$ with the same parameters.
The other halves are trained with different parameters.
We conduct through experiments on parameter sharing to show that our method is effective in Section~\ref{subsec:ablation_study}.

\subsection{Training \method}
\label{subsec:training}
\textbf{Observed data assumption.}
A latent variable $\textbf{R}_u$ represents a user's bundle interactions.
In real-world datasets, the interactions are observed as bag-of-words vectors where each element represents the counts of interactions of a user with the corresponding bundle.
We assume the vectors are drawn from multinomial distributions as in previous works~\cite{LiangKHJ18,0002WZTZ19,SankarWWZYS20,NemaKR21}, since it has shown more impressive results than other distributions such as Gaussian distributions and logistic distributions in Collaborative Filterings~\cite{LiangKHJ18}.
Bag-of-words vectors are also broadly studied in the natural language processing community~\cite{BleiNJ03}, and the vector is assumed to be sampled from a multinomial distribution owing to its remarkable performance.
Analogous to $\textbf{R}_u$, we also assume the vectors of $\textbf{X}_b$ are assumed to be drawn from multinomial distributions.

Suppose $\mathbf{R}_u$ and $\mathbf{X}_b$ are drawn from multinomial distributions as follows:
\begin{align}
\label{eq:likelihood_r_u}
	\mathbf{R}_u &\sim Mult(\sum_{b\in\mathcal{B}}{\mathbf{R}_{ub}},\pi_{\mathcal{B}}(u)),\\
	\mathbf{X}_b &\sim Mult(\sum_{i\in\mathcal{I}}{\mathbf{X}_{bi}},\pi_{\mathcal{I}}(b,u)),
\end{align}
where $Mult(N,p)$ indicates a multinomial distribution with sampling probability $p$ and the number of samplings $N$.
Note that $\pi_{\mathcal{B}}(u)$ and $\pi_{\mathcal{I}}(b,u)$ represent the probabilities of user $u$'s bundle interactions and bundle $b$'s item affiliations, respectively.
Then, the log-likelihoods of user $u$ and bundle $b$ are:
\begin{align}
\label{eq:likelihood_x_b}
	\log{p_\rho(\mathbf{R}_u|\mathbf{Z}_u)} &= \sum_{b\in\mathcal{B}}{\mathbf{R}_{ub}\log{\pi_{\mathcal{B}}(u)}}_b + C_1,\\
	\log{p_\theta(\mathbf{X}_b|\mathbf{Z}_b,\mathbf{Z}_u)} &= \sum_{i\in\mathcal{I}}{\mathbf{X}_{bi}\log{\pi_{\mathcal{I}}(b,u)_i}} + C_2,
\end{align}
where $C_1$ and $C_2$ are constants that are neglected when training parameters;
$\pi_{\mathcal{B}}(u)_b$ represents the probability of $b$'th element in $\pi_{\mathcal{B}}(u)$.

\textbf{Objective function.}
Using the log-likelihoods in Equations~\eqref{eq:likelihood_r_u} and~\eqref{eq:likelihood_x_b}, we maximize the ELBO which is stated in Equation~\eqref{eq:objective} as follows:
\begin{equation}
\label{eq:total_loss}
	\mathcal{L}_{rec} = \mathcal{L}_{mat} + \mathcal{L}_{gen},
\end{equation}
where
\begin{equation}
\label{eq:matching_loss}
\begin{multlined}
	\mathcal{L}_{mat}
	= -\frac{1}{N_u} \sum_{u\in\mathcal{U}} [\sum_{b\in\mathcal{B}} \mathbf{R}_{ub}\log{\pi_{\mathcal{B}}(u)_b}\\
	+ \frac{1}{2} (\mu_u^\top\mu_u + \sigma_u^\top\sigma_u - \log\sigma_u^\top\sigma_u)],
\end{multlined}
\end{equation}
\begin{equation}
\label{eq:generation_loss}
\begin{multlined}
	\mathcal{L}_{gen}
	= -\frac{1}{|\Omega_X|} \sum_{(u,b)\in\Omega_X} [\sum_{i\in\mathcal{I}}\mathbf{X}_{bi}\log{\pi_{\mathcal{I}}(b,u)_i}\\
	+ \frac{1}{2}(\mu_b^\top\mu_b + \sigma_b^\top\sigma_b - \log\sigma_b^\top\sigma_b)].
\end{multlined}
\end{equation}


\begin{algorithm}[t]
	\caption{Training \method}
	\begin{algorithmic}[1]
		\REQUIRE User-item interaction matrix $\mathbf{V}$, user-bundle interaction matrix $\mathbf{R}$, and bundle-item affiliation matrix $\mathbf{X}$
		\ENSURE Trained model parameters $\Theta=\{\rho, \theta, \psi, \phi\}$
%
		\WHILE {(Validation accuracy does not converge)}
			\STATE Evaluate bundle matching loss $\mathcal{L}_{mat}$ in Equation~\eqref{eq:matching_loss}
			\STATE Update parameters $\rho$ and $\psi$ to minimize $\mathcal{L}_{mat}$
			\STATE Evaluate bundle matching loss $\mathcal{L}_{gen}$ in Equation~\eqref{eq:generation_loss}
			\STATE Update parameters $\theta$ and $\phi$ to minimize $\mathcal{L}_{gen}$
		\ENDWHILE
	\end{algorithmic}
\label{alg:training}
\end{algorithm}


\textbf{Training algorithm.}
\blue{Algorithm~\ref{alg:training} presents the training algorithm of \method}.
\method is given user-item interaction matrix $\mathbf{V}$, user-bundle interaction matrix $\mathbf{R}$, and bundle-item affiliation matrix $\mathbf{X}$.
The goal of \method is to update parameters $\Theta=\{\rho, \theta, \psi, \phi\}$ minimizing the recommendation loss $\mathcal{L}_{rec}$ in Equation~\eqref{eq:total_loss}.
Specifically, \method evaluates the bundle matching loss $\mathcal{L}_{mat}$ and updates the parameters $\rho$ and $\psi$ in lines $2$ to $3$.
Then, \method evaluates the bundle generation loss $\mathcal{L}_{gen}$ and updates the parameters $\theta$ and $\phi$ in lines $4$ to $5$.
The parameter update is done until a validation accuracy converges.


